Neural Multimodal Topic Modeling: A Comprehensive Evaluation

Neural topic models can successfully find coherent and diverse topics in textual data. However, they are limited in dealing with multimodal datasets (e.g., images and text). This paper presents the first systematic and comprehensive evaluation of multimodal topic modeling of documents containing both text and images. In the process, we propose two novel topic modeling solutions and two novel evaluation metrics. Overall, our evaluation on an unprecedented rich and diverse collection of datasets indicates that both of our models generate coherent and diverse topics. Nevertheless, the extent to which one method outperforms the other depends on the metrics and dataset combinations, which suggests further exploration of hybrid solutions in the future. Notably, our succinct human evaluation aligns with the outcomes determined by our proposed metrics. This alignment not only reinforces the credibility of our metrics but also highlights the potential for their application in guiding future multimodal topic modeling endeavors.

==> old/deleted_intro.tex <==
% \begin{comment}
Overall our findings reveal that
the coherence and diversity of the topics' keywords generated by our proposed multimodal methods are similar to the one %achieved by their neural 
of their unimodal counterparts. However, the topics' overlap  between the models generated by the different approaches is rather limited. %, with subtle 
%differences %in the keyword's coherence scores 
%depending on datasets. 
Both these findings suggest that ensemble solutions should be explored. As for a direct comparison between \texttt{Multimodal-ZeroShotTM} and  \texttt{Multimodal-Contrast}, none seems to dominate the other, with the former generating more diverse textual descriptors, while the latter more coherent %textual descriptors and more 
and diverse image descriptors. This hints at the potential benefits of exploring hybrid solutions in the future.
%\ end{ comment}
%\begin{comment}
%\fg{We need to iterate over these main findings. Make it shorter and highlight the most important ones}
 \item The coherence and diversity of the topics' keywords generated by %our multimodal neural solutions are 
 Multimodal-ZeroshotTM is similar to the one achieved by its unimodal counterpart. While some of these topics  overlap between models, several of them are also unique. Our multimodal solution can be used in datasets where content is available in more than one modality to identify topics that represent the corpus better. % can be applied in datasets where content is available in more than one modality %This is encouraging, considering that these solutions can be applied in datasets where content is available in multiple modalities.
 \item We observe subtle differences in the keyword's coherence scores between Multimodal-ZeroShotTM and \texttt{Multimodal-Contrast} depending on datasets and metrics combinations. 
%\ end{ comment} 
% \begin{comment}
\begin{itemize}
\item Multimodal-ZeroShotTM can generate topics with keywords more diverse than Multimodal-Contrast. %Additionally,  even though its performance is similar to its ZeroShotTM, it produces a set of unique topics. 
Also, visualizations generated from its latent space demonstrate that  the model is able to capture the most relevant image features per topic. %Also, visualization of its latent space shows the relevance of features per each topic. 
\item On the other hand, \texttt{Multimodal-Contrast} can identify more coherence and slightly more diverse images per topic than Multimodal-ZeroShotTM. 
\item The coherence and diversity of the images selected by Multimodal-ZeroShotTM can be improved by adjusting one of its hyperparameter, however, it might affect the coherence and diversity of topics' keywords. 
\end{itemize}
% \ end{ comment}
%* Multimodal neural topic models perform similar to the unimodal counterpart. Tis is encouranging considering that it opens to new use cases. 
%* We observe subtle differences for the NPMI and $C_{v}$ scores between M3L-Contrast and Multimodal-ZeroShotTM. Depending on the metric and dataset combination, one model outperforms the other without a clear winner
%Benefits of %Multimodal-ZeroShotTM:
%% Most relevant keywords are more diverse than M3L 
%% Even thought their topic's coherence and diversity is similar to ZeroShotTM, we demostrate that it can produces unique topics compared with their unimodal counter part (this is good). 
%% We demostrate that by reconstructing image features, the model can capture relevant features per each topic. (explain how). 
%%We also demostrate that by adjusting the weigh of the image reconstruction loss, the image coherence and diversity can improve, but it may sacrifice keyword's coherence and diversity. 
%Benefits of %Multimodal-Contrast:
%% Most relevant images shared more relatedness (higher IEC score) than Multimodal-ZeroShotTM
%% Slight more image diversity (i-EPS score)
%%
%which makes it more efficient than M3L-Contrast. 
 %   We propose a quantitative approach to assess the coherence and diversity of the top \textit{N} images that describe a topic   
 %    We conduct a comparative study of two neural topic modeling algorithms over six datasets from different domains and with different characteristics.   
    %\item We make available (upon acceptance oft this paper) a set of ...
     %$$\item %We present a neural multimodal topic model. We show that reconstructing BoW and image embeddings generates more coherent and diverse topics than a state-of-the-art model
% \end{itemize}
% \ begin{comment}
We summarize prior work on topic modeling in Section \ref{sec:related_work}. Section \ref{sec:proposal} introduces MultiModalZeroShotTM and the adaption of M3L-Contrast to make it multimodal-only. Section \ref{sec:experiments}  details our comparative study of these two neural topic models, while Section \ref{sec:results} reports on our findings. Section \ref{sec:discussion} offers a discussion of our results, limitations, and future work. Finally, Section \ref{sec:conclusions} provides our conclusions. 
\end{comment}
%M3L-Contrast~\cite{zosa2022multilingual} is a recent multimodal multilingual neural topic model that uses Contrastive learning to map texts from multiple languages and images into a shared topic space. By being both multilingual and multimodal,  it can identify aligned language-specific topics and infers textual representations of semantic concepts in images. However, this model can only be used in datasets where a document comprises three components: a text in one language, a text in a second language, and an image. 
  

%M3L-Contrast includes three inference networks, one per modality and language, increasing the model's time and space complexity. In addition, while it aims to capture information from images using a contrastive learning loss, the decoders only reconstruct elements associated with the documents' textual component (bag-of-words) but nothing related to the images. As a result, the model might not capture all the information contained in the documents and not fully understand the relationship between the text and image.

%Considering previous limitations, in this work, we modify M3L-Contrast to allow its use in more generic multimodal datasets, where a document is composed by an (image, text) pair. We also introduce MultimodalZeroShotTM, a neural multimodal topic model that uses pre-trained textual and image embeddings to identify coherence and diverse topics. Our approach involves a unique inference network,  which makes it more efficient than M3L-Contrast. Moreover, the decoder reconstructs data associated with the textual and visual components from the documents, their bag-of-words, and image features, respectively. These approaches help the model capture relevant information from the images and can make the model generate topics that better represent the corpus. 

%and understand the relationship between the textual and visual components of the document. 

%Considering previous limitations, in this work, we modify M3L-Contrast to allow its use in more generic multimodal datasets, where a document is composed by an (image, text) pair. We also introduce MultimodalZeroShotTM, a neural multimodal topic model that uses pre-trained textual and image embeddings to identify better topics. Our approach involves a unique inference network,  which makes it more efficient than M3L-Contrast. The decoder also reconstructs the bag-of-words and image features during the loss computation. \fg{Explain the benefit of that}




%Our work introduces a neural multimodal topic model that utilizes pre-trained document and image embeddings to simplify the complexities that arise from multiple modalities. Our work is based on CTM, a family of topic models that use pre-trained representations of language (e.g., BERT) to support topic modeling. 

%Our work is based on the contextualized topic model (CTM), a family of topic models that used contextualized document


%In this work, we present a neural multimodal topic model that takes advantages of pretrained document and image embeddings to abstract the complexities between languages and modalities. 


%The majority of topic modeling algorithms have been designed to process textual data only. However, nowadays, data appears in different modalities. For example, social media users post content either by text, image, or both~\cite{9696359}. 

%(e.g., social media users posting content either by text, images or both 



%Most toopic models are designed for textual data, but there is work on applying topic modeling to (text, images) as well.. 

%Topic model focusing only on textual data may pick different topics for such documents~\cite{9696359}

%However, data nowadays are available in multiple modadalities (e.g., people express themselves on social media either by using text, images, or both~\cite{9696359})

%why multimodal? Find relantionship between text and images. Find more comprehensiveness topics? 
%Documents can have similar images but completely different textual content ~\cite{9696359}
%Incorporating another level of information (e.g., images) might help to models to identify more comprehensive topics~\cite{9696359}

%Applications

%Brief summary of neural topic models

%
%To deal with multimodal data, some variants of LDA have been proposed (see here
%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=6909574)


%M3L Contrast, there is multilingual and multimodal.%Explain that we remove one of the component to make it multimodal only.

%Also, we present an alternative model. MultimodalZeroShotTM, which ... do this to ... to dat. %We believe that the reconstruction of images may help to produce high-quality topics. 

%We show that .. 

%In this work we present 
%\fg{Problem description is missing here}


%Multimodal modeling is the main solution for modelign image and tex modalities simultaneously into a univerm lmodel. ~\cite{6971080}


%\descr{Focus \& Research Questions.} 
%This work focuses on ....
%Specifically,  we focus on shedding light on the following research questions:

%\begin{itemize}
    %\item \textbf{RQ1:} 
    
    %\item \textbf{RQ2:} 

%\end{itemize}


%Our work is based on the contextualized topic model (CTM), a family of topic models that used contextualized document


%In this work, we present a neural multimodal topic model that takes advantages of pretrained document and image embeddings to abstract the complexities between languages and modalities. 


==> sections/05_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\begin{comment}
    

\fg{These are ideas that might be included in the discussion}
\begin{itemize}
    \item \sout{Explain why the performance of ZeroShotTM is very similar to Multimodal-ZeroShotTM. }
    \item \sout{New use cases of $\gamma$ (latent space in MultimodalZeroShotTM). Explain the benefit of reconstructing images over Multimodal-Contrast. (e.g., topic labeling)}
    \item \sout{Explain why \texttt{Multimodal-ZeroShotTM} always generates more diverse topics}
    \item \sout{Try to explain why \texttt{Multimodal-Contrast} performs better in terms of IECO score}
    \item \sout{Explain differences between datasets that might impact the results (e.g., doc length)}
    \item \sout{Why Multimodal algorithms are relevant/needed (even if they get the same or worse  performance than unimodal)}
    \item \sout{Trade-off for coherence/diversity for different $\lambda$}
    \item  \sout{Explain why \texttt{Multimodal-Contrast} performs worse than ZeroShotTM}
    \item \sout{RQ: Wha method works better on which dataset.} 
    \item \sout{What evaluation metrics are more appropriate in the new multimodal scenario}
    \item \sout{why images are relevant (as topic descriptors, it helps for topic interpretation). I can cite my topicvisexplroer paper. }
\end{itemize}
%\fg{In the discussion section, I will describe all the ideas that came to my mind. Then, we need to filter those}

\end{comment}
%\descr{Multimodal neural topic models perform similarly to its unimodal counterpart}. We identify that \texttt{Multimodal-ZeroShotTM} and \texttt{Multimodal-Contrast} generates topics, with keywords similar coherent and diverse that their unimodal counterpart, ZeroShotTM. 

Our study evaluates topic modeling techniques on datasets representing documents by image and text pairs. We identify the quality of the resulting topics in terms of their coherence and diversity. We propose two new metrics to measure the coherence and segregation of images representing topics. We also offer a new benchmark for multimodal topic modeling. Our experiments lead to several findings. We discuss the implications of them below. 


%Our study evaluates topic modeling techniques on datasets where documents are represented by (image, text) pairs. We identify the quality of the resulting topics in terms of their coherence and diversity. We use well-established automatic metrics to analyze the quality of the most relevant keywords per topic. Given that we are also interested in the quality of the top relevant images per topic, we adapt metrics from the state of the art to fill this gap. Our experiments lead to several findings. We discuss the implications of them below. 

%Our study focuses on evaluating topic modeling techniques on datasets where documents are represented by (image, text) pairs. We identify the quality of the resulting topics in terms of their coherence and diversity. To do so, we use well-established automatic metrics designed to analyze the most relevant keywords per topic. Given that we are also interested in the quality of the top relevant images per topic, we adapt metrics from the state of the art to fill this gap. Our experiments lead to several findings, we discuss the implications of them below. 


Overall, we identify that \texttt{Multimodal-ZeroShotTM} %and Multimodal-Contrast
generates topics with similar quality to those generated by their unimodal counterpart, ZeroShotTM.  While there is some overlap for some topics generated by these models, they also produce a set of unique topics. %This is measured regarding the coherence and diversity of the most relevant keywords per topic. 
This is encouraging, considering that the \texttt{Multimodal-ZeroShotTM} allows extracting topics from datasets where text and image content coexist and need to be analyzed jointly. %Our intuition is that by capturing relevant aspects from both modalities, topic models can extract more meaningful and semantic corpus representations.  %content is available in textual and visual modalities (e.g., image and its caption). Considering both modalities, multimodal neural topic models might extract more meaningful and semantic corpus representations.  
Each modality captures different aspects of information, and they complement each other~\cite{roller2013multimodal}. By integrating both modalities, multimodal neural topic models can  extract more meaningful and semantic corpus representations than their monolingual counterparts~\cite{6971080}. 


%By integrating both modalities,  our intuition is that neural topic models can  extract more meaningful and semantic corpus representations. %provide topics that are more meaningful and more represenative
%\fg{Topic's overlap}

Our proposed models can benefit users in different ways. For instance, with Multimodal-Contrast, which incorporates two inference networks (one per modality), users can identify topic distributions from documents available in a single modality (e.g., a set of images without any accompanying caption). This capability is achieved after training the model on text and image pairs. %Inferring topic distributions of unseen documents is a common practice among researchers of different areas (e.g., social science).


%Our proposed models can benefit users in different ways. For example, given that \texttt{Multimodal-Contrast} contains two separate inference networks, once the model is trained on (text, image) pairs, users can infer topic distribution from documents available in one modality only (e.g., an image without any caption). Inferring topic distributions of unseen documents is a common practice among researchers of different areas (e.g., social science). %On the other hand, 
%\texttt{Multimodal-ZeroShotTM} requires documents with both components (i.e., textual and visual parts) during inference, given that its architecture includes a unique inference network. 


%\texttt{Multimodal-ZeroShotTM} incorporates a topic image-feature matrix  $\gamma$, that captures relevant image features for each topic. This matrix holds potential for several NLP tasks. For example, in existing visual and multimodal classification tasks, introducing it as an additional input might enhance classification accuracy. Furthermore, it could be utilized in document similarity tasks, where the relatedness between this component and documents can be measured. 

%MENTION IN FUTURE WORK

%\texttt{Multimodal-ZeroShotTM} incorporates a topic image-feature matrix  $\gamma$, that captures relevant image features for each topic. This matrix could be valuable in several NLP tasks. For example, introducing it as an additional input might enhance classification accuracy in existing visual and multimodal classification tasks. In the same way, it might improve the performance of document similarity tasks. Additionally, we anticipate a  potential utility of the topic image-feature matrix for topic labeling tasks, given that the images generated by the CLIP-Guided Diffusion model strongly align with the topics' descriptors. Future work should assess how much these generated images can help during topic interpretation and evaluation. 


%We demonstrate that \texttt{Multimodal-ZeroShotTM} can capture relevant image features per topic, stored in the $\gamma$, a topic image-features matrix. We anticipate some potential use cases of $\gamma$ for NLP tasks. For instance, current text and visual classification tasks could receive $ \gamma $ as an additional input, potentially improving their classification accuracy. Moreover, it could also be used for document similarity tasks, where the relatedness between this matrix and documents (either its textual or visual component) can be measured. 


%We reconstruct an image per topic using a CLIP-Guided Diffusion model over $\gamma$. The resulting images are well-aligned with the topic's keywords, and they are very descriptive. This opens the door to using this or similar approaches for automatic topic labeling, which can facilitate the interpretation of topics. % and facilitating the interpretation of topics. 

%We also see the potential of using the topic image-feature matrix for topic labeling tasks, as the generated images from the CLIP-Guided Diffusion model were very highly aligned with the topics' descriptors. Future work should assess how much it can help during topic interpretation and topics evaluation. 



%We reconstruct an image per topic using a CLIP-Guided Diffusion model over $\gamma$. The resulting images are well-aligned with the topic's keywords, and they are very descriptive. This opens the door to using this or similar approaches for automatic topic labeling, which can facilitate the interpretation of topics. % and facilitating the interpretation of topics. 

NOY AN EXPLANATION
The differences in performances between \texttt{Multimodal-ZeroShotTM} and \texttt{Multimodal-Contrast} could be explained by their differences in integrating information from textual and visual modalities. For instance, our evidence suggests that mapping between vectors from different modalities by contrastive learning loss leads to a narrower range of keywords, while  %On the other hand, 
reconstructing both BoW and Image Features %during training 
allows the model to capture a more comprehensive variety of visual aspects, leading to a more diverse representation of topics' keywords.

%The mechanisms that both \texttt{Multimodal-ZeroShotTM} and \texttt{Multimodal-Contrast} use to integrate information from textual and visual modalities differ, resulting in different performances. We observe that \texttt{Multimodal-Contrast} cannot generate topics' keywords as diverse as those selected by Multimodal-ZeroShotTM.  While the reasons for it require further investigation, our intuition is that the mapping between vectors from different modalities by the contrastive learning loss leads to a narrower range of keywords. On the other hand,  \texttt{Multimodal-ZeroShotTM} might be able to identify a more comprehensive variety of visual aspects that lead to a more diverse representation of topics' keywords.

%In the same way, we identify differences in the coherence and diversity of the top images per topic. Across all datasets, the images per topic selected by \texttt{Multimodal-Contrast} have more relatedness than those chosen by Multimodal-ZeroShotTM. At the same time, the selected images per \texttt{Multimodal-Contrast} are more diverse between topics. Lower redundancy between topics can help humans to distinguish the nuances between them and support their interpretation. 

The performance of models might also be affected by the datasets' properties. For instance, \texttt{Multimodal-ZeroShotTM} shows higher NPMI and $C_{v}$ scores in documents with fewer keywords (six to ten words). 

MOST OF THIS IS JUST SPECULATION... CUT?
In addition, the domain and content of the datasets also play a role. For example, suppose a dataset focuses more on visual aspects (e.g., an image captioning dataset as MS COCO). In that case, the best multimodal neural topic model might be the one that can generate topics' descriptors highly associated with relevant image features. Finally, the source and data collection process is also relevant. For example, data collected from social media platforms can exhibit different properties than those gathered from scientific publications or news articles. At the same time, how data is collected or annotated can introduce biases (i.e., depending on annotation quality or data imbalance) that can affect the performance of models. 



%The subtle differences between \texttt{Multimodal-ZeroShotTM} and \texttt{Multimodal-Contrast} in terms of NPMI and $C_{v}$ scores might be attributed to several factors, including document characteristics. For example, \texttt{Multimodal-ZeroShotTM} shows performance better than \texttt{Multimodal-Contrast} when the textual content is short (six to ten words). 

%The domain and content of the datasets might explain other differences. Each corpus represents a particular domain and reveals variations in the distribution of topics. For example, MS COCO is an image captioning dataset, while  T4SA is a sentiment analysis dataset. The variation in content can impact the ability of the models to capture coherent and diverse topics. 

%The source and data collection process can also explain the difference between models. For example, one model might deal better with crowdsourced datasets (e.g., MS COCO and MEWA datasets), which might exhibit some subjectivity. In contrast, other models might be better at dealing with datasets originating from a mix of human and automatic intervention (e.g., HC-4chan) from social media (i.e., 4chan). 




%For example, one model might deal better with crowdsourced datasets (e.g., MS COCO and MEWA datasets), which exhibit some subjectivity. In contrast, other models might better deal with datasets from a mix of human and automatic interventions (e.g., HC-4chan).


%The source and data collection process can also explain the different performances. For example, one model might deal better with crowdsourced datasets (e.g., MS COCO and MEWA datasets), which exhibit some subjectivity. In contrast, other models might better deal with datasets from a mix of human and automatic interventions (e.g., HC-4chan).

%CUT ? GIVEN THAT WE PUT LAMBDA IN THE APPENDIX

%We identify that by attributing more weight $\lambda$ to the image feature reconstruction loss, MultimodalZeroShotTM can identify more coherent and diverse topics. However, the coherence and the diversity of the topics' keywords are slightly affected. Several factors might explain this behavior. First, higher values of $\lambda$ make the model focus more on identifying visual patterns and relationships between image features leading to a better representation of visual concepts within the topics. However, a higher value does not explicitly enforce the model to capture better the relationship between topics' keywords. Textual and image have different structures and semantics, resulting in a trade-off between visual and textual topics' coherence and diversity. 

%IN CONCLUSIONS
%To the best of our knowledge, no prior work focused on evaluating image coherence and diversity for multimodal topic modeling algorithms. This work provides researchers and practitioners with a comprehensive toolkit for assessing neural topic models regarding image-topic associations. Our metric \texttt{IEC} quantitatively assesses visual consistency within topics. Furthermore, our metric \texttt{IEPS} addresses the need for diverse image representations between topics, which is crucial to avoid redundancy and ensure a richer exploration of the corpus. 

%ALSO IN INTRO OR CONCLUSIONS
%We also highlight the relevance of including images as topic descriptors, as they are valuable in multiple ways. They offer complementary levels of information and context that might not be explicitly in the top keywords per topic. Images can also provide more fine-grained details about the semantics of the topic and encapsulate abstract concepts. When the relationship between keywords is unclear (e.g., noisy keywords), observing the most relevant images per topic might be easier to interpret. 


%We anticipate that topics with high image coherence and diversity will help during topic interpretation. Considering images as topic descriptors are valuable in multiple ways. They offer complementary levels of information and context that might not be explicitly in the top keywords per topic. Images can also provide more fine-grained details about the semantics of the topic. When the relationship between keywords is not clear (e.g., noisy keywords), observing the most relevant images per topic might be easier to interpret. 


%Having images as topic descriptors is valuable in several ways. First they can offer complementary information, capture fine-grained details and context that is not explicity in the top keywords per topic. When the relantionship between keywords is not clear (e.g., noisy keywords), images might eb more easy to interpret and intuitive. 


%First, they can reveal complex pattern, uncover hidden connections, offer complementary information, 


%%bridge the gap insights more effectively, unravel complext patterns, uncover hidden connections. 
%% images - topic descriptors, aid topic interpretation. More intuitite and easily interpretable than keywords alone (especially if the keywords do not provide much information by itself or there are noisy keywords). Offer complementary information, capture fine grained details, and context that not might be expressed in the top ten words per topic. They can capsule complex and abstract concepts, and engage users in topic interpretation. 
%%
%% 

%%

%In the multimodal scenario, well-established topics' coherence and diversity metric 


%
%To the best of our knowledge, there is no prior work focused on  the evaluation of image coherence and diversity for multimodal topic modeling algorithms. In this work, we provide researchers and practitioners with a comprehensive toolkit to evaluate neural topic models in terms of image representation. Our metric \texttt{IEC}, provides a quantitative assessment of visual consistency within topics and allows to get insights into the  image-topics associations. Our metric \texttt{IEPS}, address the need for diverse images representations between topics, which is crucial to avoid redundancy and get a richer exploration of the content. 

%%**
%%Fill the gap, there is no automatic prior work focused on image coherence and diversity evaluation for multimodal topic modeling
%researchers and practitioners, comprehensive tooltik, to evaluate the perfromance of multimodal models, in terms of image representation. 
%They can get a better understanding of how well topics align with visual content,  and how %%Coherence of topic ---> contribution: quantitative assessment of visual consistency withing tpics, insights quality generated image topic association.
%%Diversity: Our diversity metric -> address the need for diverse image representation across topics. Avoid redundancy, richer exploration of visual content. 



%We identify that by attributing more weight $\lambda$ to the image feature reconstruction loss, MultimodalZeroShotTM can identify more coherent and diverse topics. However, the coherence and the diversity of the topics' keywords are slightly affected. Several factors might explain this behavior.  Higher values of $\lambda$ make the model focus more on identifying visual patterns and relationships between image features leading to a better representation of visual concepts within the topics. However, higher values of $\lambda$ do not explicitly enforce the model to capture better the relationship between topics' keywords. Textual and image have different structures and semantics. This semantic gap between modalities results in a trade-off between visual topic coherence and diversity and textual topic coherence and diversity. 


%%textual image different structure semantics, %higher value this not explicitly enforce the coherence and diversity of keywortss. %The semantic gap between modalities result ina  trade off between visual topic coherence and diversity. 




%%data collection, can introduce biases, 

%%






%%%

%%%

%In the same way, we identify differences in the coherence and diversity of the top images per topic. Across all datasets, \texttt{Multimodal-Contrast} shows that it can  identify the group of images with more relatedness than those selected by Multimodal-ZeroShotTM. At the same time, the first model is able to generate topics with more distinct images between topics. 


%The mechanisms that both \texttt{Multimodal-ZeroShotTM} and \texttt{Multimodal-Contrast} integrate information from textual and visual modalities differ and therefore result in different performances.  We observe that \texttt{Multimodal-Contrast} is not able to generate topics' keywords as diverse as those selected by Multimodal-ZeroShotTM.  While the reasons for it require further investigation, our intuition is that the mapping between vectors from different modalities by the contrastive learning loss leads to a narrower range of keywords. \texttt{Multimodal-ZeroShotTM} might be able to identify a variety of visual aspects that lead to a more diverse representation of topics' keywords.  %On the other hand, \texttt{Multimodal-ZeroShotTM} 


%ultimodal-Contrast may have a different strategy or weighting scheme for combining text and image information, leading to a narrower range of keywords generated for topics. Multimodal-ZeroShotTM, with its emphasis on image feature reconstruction, may capture a wider variety of visual aspects that contribute to more diverse keyword representations


%\fg{Need to finish this section}.
%\texttt{Multimodal-ZeroShotTM} can generate topics with more coherent and diverse keywords than \texttt{Multimodal-Contrast} while maintaining a level of coherence similar to ZeroShotTM. This suggests that the model is able to capture aspects of every modality to produce a more distinct list of topics, which we


%\texttt{Multimodal-ZeroShotTM} can generate topics with more coherent and diverse keywords than \texttt{Multimodal-Contrast} while maintaining a level of coherence similar to ZeroShotTM. This suggests that the model is able to capture aspects of every modality to produce a more distinct list of topics, which we

%This suggests that the model can leverage content from both modalities to produce  more comprehensive topics.  %This suggests that the model can leverage content from both modalities to produce topics,  which might be more comprehensive and representative of the corpus. 


%\fg{Need to finish this paragraph and section}










%\fg{Talk that \texttt{Multimodal-Contrast} loose performance over zeroshottm. Our proposal Multi-contrast does not loose performance, is the same. Also, it can have more applications!!}

%\fg{I could use visualize latent space for topic labeling}
%\fg{Explain and justify how the performance of Multimodal-zEROSHOT TM is equal to zeroshottm? is really learning?}
%\fg{\texttt{Multimodal-Contrast} always generate more diverse topics}
%\fg{Try to explain why \texttt{Multimodal-Contrast} perform better in terms of IECO scores}
%\fg{Maybe the lenght of the document is a difference. A model perform better than the other why? it can capsule more ?}
%\fg{Explain why if we dont improve the performance of unimodal, why we care still about this?}
%
%\fg{Mention benefits of using Multimodal over zeroshottm (even if we get worse performance)}

%\fg{Explain why the performance of the model decreases after injecting images}


%\fg{We can improve the coherence of the images by increasing lambda, but we decrease the performance of the keywords.}




%\fg{Mention that we also have results with MSE loss, the overall results do not change}
%
%\subsection{Features reconstruction}



%\fg{Explain the motivation of why reconstructing make sense (that should be in the methodology as well)}

%\fg{Explain the results - The tradeOFF}



\begin{comment}
\begin{table*}[ht]
\setlength{\tabcolsep}{2pt}
\centering
%\resizebox{\textwidth}{!}{%
\footnotesize
\begin{tabular}{lrrrr|rrrr|rrrr|rrrr|rrrr|rrrr}
\toprule
\multicolumn{1}{c}{Dataset} &
  \multicolumn{4}{c}{VIST} &
  \multicolumn{4}{c}{MS COCO} &
  \multicolumn{4}{c}{4chan} &
  \multicolumn{4}{c}{MMHS150} &
  \multicolumn{4}{c}{T4SA} &
  \multicolumn{4}{c}{WIT} \\
  \midrule
\multicolumn{1}{c}{Metrics} &
  \multicolumn{1}{|c}{$\tau$} &
  \multicolumn{1}{c}{$\phi$} &
  \multicolumn{1}{c}{$\alpha$} &
  \multicolumn{1}{c}{$\gamma$} &
   \multicolumn{1}{|c}{$\tau$} &
  \multicolumn{1}{c}{$\phi$} &
  \multicolumn{1}{c}{$\alpha$} &
  \multicolumn{1}{c}{$\gamma$} &
   \multicolumn{1}{|c}{$\tau$} &
  \multicolumn{1}{c}{$\phi$} &
  \multicolumn{1}{c}{$\alpha$} &
  \multicolumn{1}{c}{$\gamma$} &
   \multicolumn{1}{|c}{$\tau$} &
  \multicolumn{1}{c}{$\phi$} &
  \multicolumn{1}{c}{$\alpha$} &
  \multicolumn{1}{c}{$\gamma$} &
   \multicolumn{1}{|c}{$\tau$} &
  \multicolumn{1}{c}{$\phi$} &
  \multicolumn{1}{c}{$\alpha$} &
  \multicolumn{1}{c}{$\gamma$} &
  \multicolumn{1}{|c}{$\tau$} &
  \multicolumn{1}{c}{$\phi$} &
  \multicolumn{1}{c}{$\alpha$} &
  \multicolumn{1}{c}{$\gamma$}  \\ 
  \midrule

\multicolumn{1}{l|}{BoW} &
  &
   &
   &
   &
   &
  &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\

\multicolumn{1}{l|}{BoW + Image features} &
  &
   &
   &
   &
   &
  &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
   
\multicolumn{1}{l|}{BoW + Text features} &
  &
   &
   &
   &
   &
  &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
   
\multicolumn{1}{l|}{BoW + Img features + Text features} &
  &
   &
   &
   &
   &
  &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\
  \bottomrule
\end{tabular}
%}
\caption{Coherence scores of the top keywords and images. We used the following abbreviations: NPMI ($\tau$), $C_{v}$ ($\phi$), WECO ($\alpha$), and IECO ($\gamma$).  Average results over $4$ number of topics ($K = 25, 50, 75, 100$), where the results for each $K$ are averaged over $30$ random seeds. We bold best values }
\label{tab:ablation_study_results_per_dataset}
%\vspace{-.5em}
\end{table*}


\end{comment}
